Non-reciprocal frequency conversion in a multimode nonlinear system

Nonlinear optics has become the workhorse for countless applications in classical and quantum optics, from optical bistability to single photon pair generation. However, the intrinsic weakness of optical nonlinearity has meant that large input powers and weak output powers are often a necessity in nonlinear frequency conversion. Here, motivated by recent advances in using non-Hermitian photonics and gain/loss engineering to enable non-reciprocal light transport, we explore how the interplay between non-Hermiticity and optical nonlinearity leads to a fundamentally new regime of nonlinear frequency conversion. We show how non-Hermitian coupling between discrete frequency modes can result in non-reciprocal flow of energy in the frequency dimension, closely resembling the non-Hermitian skin effect (NHSE). Applying our theory to a multimode nonlinear cavity supporting cascaded nonlinear processes, we create an asymmetric infrared (IR) comb that features a ``skin'' frequency mode populated with efficiency exceeding 85\%. Furthermore, we demonstrate how three-wave mixing processes in the non-reciprocal infrared comb we generate enables terahertz (THz) generation exceeding the Manley-Rowe limit. We then show how the non-reciprocal frequency conversion is robust against cavity defects and disorder that cause random fluctuations in the dissipation rate for different modes. Moreover, in certain regimes, the nonlinear, non-Hermitian system supports stable limit cycles that can enable multimode pulsing with picosecond pulse widths and GHz repetition rates. Finally, we explore how the system can be applied to generate simultaneous IR and THz frequency combs, potentially unlocking novel applications in spectroscopy and metrology.

==> preamble.tex <==
%-----CHANGING CITATION APPEARANCE----
\setcitestyle{numbers,square,sort&compress} %We don't want the rmp citation style, but standard style square bracket, numbers style instead

%----KERNING-----
\usepackage{microtype} %For better kerning and symbol-stretching
\usepackage{xspace} %For the \xspace command

%----LOADING RELEVANT FONTS [TIMES ROMAN FOR PRB] -----
\usepackage{txfonts}  %Times Roman fonts
\usepackage{txfontsb} %Addition for txfonts, including old style numerals and greek
%					  %\usepackage{mathptmx} Also a Times Roman Font
%\usepackage{bm} %Bold math symbols with \bm{} (Greek and other symbols)
%\usepackage{mnsymbol} %For llangle and rrangle

%-----CROSS-REFERENCING-----
\usepackage{xr}

%-----COLOR AND GRAPHICS PACKAGES-----
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{calc,decorations.markings}

%-----SETTINGS FOR REFERENCES-----
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={blue!75!black!80!yellow},
    citecolor={blue!75!black!80!yellow},
    urlcolor={blue!75!black!80!yellow}
}

%-----PACKAGE FOR BOXED MULTI-LINE EQUATIONS-----
\usepackage{empheq}
\newcommand*\widefbox[1]{\fbox{\hspace{2em}#1\hspace{2em}}}

%-----CHANGE MARGINS OF DOCUMENT-----
\usepackage[top=1in, bottom=1.5in, left=1.4in, right=1.4in]{geometry} %Change margins

%-----SOME SETTINGS FOR MARGINPAR-----
%\usepackage{marginfix} %Should fix even more than mparhack, so use this instead unless you see something funky

\let\oldmarginpar\marginpar %This and the next line changes the fontsize
\def\marginpar#1{\oldmarginpar{\scriptsize #1}}
\setlength{\marginparwidth}{6.5em} %Changes the width of the note
\setlength{\marginparsep}{2em} %Probably enforces a minimum distance between marginpar-notes


%INCLUDING CLEVEREF PACKAGE FOR MORE CONVENIENT REFERENCING ABILITIES
\usepackage[capitalize,nameinlink]{cleveref}
\newcommand{\crefrangeconjunction}{\,--\,}
\crefname{subequations}{Eqs.}{Eqs.} %Specific changes to allow for Eqs.-wording when referring to a set of subequations. Label of subequations must include [subequations] as an option.
\Crefname{subequations}{Eqs.}{Eqs.}
\crefformat{subequations}{#2Eqs.~(#1)#3}
\Crefformat{subequations}{#2Eqs.~(#1)#3}
\crefname{page}{p.}{p.} %Changing from 'page' to 'p.'
\newcommand{\heqref}[1]{\hyperref[#1]{(\ref*{#1})}} %Alternative to \eqref, which works better with hyperlinks (whole thing is clickable)
\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable
\newcommand{\namedeqref}[2]{\hyperref[#2]{#1~(\ref*{#2})}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable


%-----PACKAGE TO ALLOW CHANGING OF ENUMERATE BULLETS-----
\usepackage{enumitem}

%-----COMMANDS-----
\newcommand{\vek}[1]{\mathbf{#1}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\nablav}{\boldsymbol{\nabla}}
\newcommand{\hxv}{\hat{\mathbf{x}}}
\newcommand{\hyv}{\hat{\mathbf{y}}}
\newcommand{\ef}{\epsilon_{\text{\textsc{f}}}}
\newcommand{\vf}{v_{\text{\textsc{f}}}}
\newcommand{\tsc}[1]{\text{\textsc{#1}}}
\newcommand{\kb}{k_\tsc{b}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ddb}[1]{\!\dd#1\,}
\newcommand{\dde}{\,\dd}
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern.2pt}\sim\cr\noalign{\kern-2.5pt}}}}}

\newcommand{\spar}{_{\scriptscriptstyle\parallel}}
\newcommand{\kpar}{k_{\scriptscriptstyle\parallel}}
\newcommand{\kvpar}{\kv_{\scriptscriptstyle\parallel}}
\newcommand{\rpar}{r_{\scriptscriptstyle\parallel}}
\newcommand{\rvpar}{\rv_{\scriptscriptstyle\parallel}}
\newcommand{\vpar}{v_{\scriptscriptstyle\parallel}}
\newcommand{\vvpar}{\vv_{\scriptscriptstyle\parallel}}
\newcommand{\dperp}{d_{\perp}}
\newcommand{\dpar}{d_{\parallel}}
\newcommand{\iu}{\mathrm{i}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\sgn}{\operatorname{sgn}}

\newcommand{\pr}[1]{|#1\rangle\langle#1|}
\newcommand{\prsf}[1]{\mathsf{|#1\rangle\langle#1|}}

\newcommand{\Ev}{\mathbf{E}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Hv}{\mathbf{H}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\dv}{\mathbf{d}}
\newcommand{\hv}{\mathbf{h}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\Gv}{\mathbf{G}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\nv}{\hat{\mathbf{n}}}

%abbreviations
\newcommand{\ie}{i.e.\@\xspace} %Gobble-spaces of the "small" type (small is ensured by adding \@)
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
